Graphsurge: Graph Analytics on View Collections Using Differential Computation

This paper presents the design and implementation of a new open-source view-based graph analytics system called Graphsurge. Graphsurge is designed to support applications that analyze multiple snapshots or views of a large-scale graph. Users program Graphsurge through a declarative graph view definition language (GVDL) to create views over input graphs and a Differential Dataflow-based programming API to write analytics computations. A key feature of GVDL is the ability to organize views into view collections, which allows Graphsurge to automatically share computation across views, without users writing any incrementalization code, by performing computations differentially. We then introduce two optimization problems that naturally arise in our setting. First is the collection ordering problem to determine the order of views that leads to minimum differences across consecutive views. We prove this problem is NP-hard and show a constant-factor approximation algorithm drawn from literature. Second is the collection splitting problem to decide on which views to run computations differentially vs from scratch, for which we present an adaptive solution that makes decisions at runtime. We present extensive experiments to demonstrate the benefits of running computations differentially for view collections and our collection ordering and splitting optimizations.

==> aggregate-views.tex <==
\section{Aggregate Views}\label{subsec:aggregate-views}
We are implementing \graphsurge{} to be a full-fledged view-based graph analytics system. To allow a wider range of applications to be developed on the system, we support {\em aggregate views}, which are views introduced in the Graph OLAP literature~\cite{chen:graph-olap, zhao:graph-cube}. An aggregate view over an input graph $G$ describes a particular high-level connectivity summary of $G$. Specifically, aggregate views group sets of nodes in $G$ into super-nodes and aggregate the original edges between nodes into super-edges, with the semantics that each edge $(u, v)$ in the original graph becomes part of an aggregation of a super-edge between the super-nodes that $u$ and $v$ belong to. GVDL contains group by constructs on nodes to define super-nodes, and aggregate constructs on nodes and edges to define aggregate properties on super-nodes and super-edges. The resulting query is evaluated in TD using a dataflow that consists of aggregation operators. 

\begin{example}\label{ex:aggregated-view} 
{\em
Listing~\ref{lst:agg-views} shows two aggregate views. The first is an aggregate view showing the total calls made between doctors in NY, lawyers in LA, and teachers in DC (so a triangle). The second is the city-calls-city view
that captures the connectivity of calls between cities, where city super-nodes have a \texttt{num-phones} property, for the number of phone calls registered in the city, and super-edges have a \texttt{total-duration} property for the total duration of calls made between cities.
}
\end{example}

\begin{lstlisting}[float,
    caption={Example GVDL aggregate view queries.},
    label={lst:agg-views}, belowskip=-0.8 \baselineskip]
create view NY-Dr-CA-Lawyer on Calls
nodes group by [
        (profession=`Doctor' and city=`NY'),
        (profession=`Lawyer' and city=`LA'),
        (profession=`Teacher' and city=`DC')]
      aggregate count(*)
create view City-Calls-City on Calls
nodes group by city aggregate num-phones: $\textbf{count}$(*)
edges aggregate total-duration: $\textbf{sum}$(duration)
\end{lstlisting}
Supporting aggregate views allows users to start analytics on very large graphs, construct smaller graphs by creating aggregate views, and perform further graph analytics on these smaller graphs, all in the same system. We plan to extend the system with new features as we encounter other view-based graph analytics applications. 

